Data Diversity as Implicit Regularization: How Does Diversity Shape the Weight Space of Deep Neural Networks?

Data augmentation that introduces diversity into the input data has long been used in training deep learning models. It has demonstrated benefits in improving robustness and generalization, practically aligning well with other regularization strategies such as dropout and weight decay. However, the underlying mechanism of how diverse training data contributes to model improvements remains unknown. In this paper, we investigate the impact of data diversity on the weight space of deep neural networks using Random Matrix Theory. Through spectral analysis and comparing models trained with data augmentation, dropout, and weight decay, we reveal that increasing data diversity alters the weight spectral distribution similarly to other regularization techniques, while displaying a pattern more closely aligned with dropout than with weight decay. Building on these insights, we propose a metric to explain and compare the benefits of diversity introduced by traditional data augmentations and those achieved through synthetic data.

==> sections/3.1SynData.tex <==
What kind of training data do we need or beneficial for a robust



==> sections/note.tex <==
The model performance, including prediction accuracy or calibration error, is impacted by two factors: input data and model structure. For the pretrained model, the model weights and specific fine-tuning datasets would both determine the model performance. 

Random Matric Theory: 
The more information the model learns, the less random weight matrices would be.



The λmax is a measure of the size, or scale, of W 









-----------------backup 

\textcolor{blue}{These charts show the relative changes of $\Delta M$ compared to the baseline. We observe that three of four metrics have the same trend for all regularization and data augmentation methods. Abbreviations ``dp'', ``wd'' and ``div'' denote dropout, weight decay, and data augmentation, respectively.} \textcolor{blue}{remove}

